On Universality in Human Correspondence Activity

Identifying and modeling patterns of human activity has important ramifications in applications ranging from predicting disease spread to optimizing resource allocation. Because of its relevance and availability, written correspondence provides a powerful proxy for studying human activity. One school of thought is that human correspondence is driven by responses to received correspondence, a view that requires distinct response mechanism to explain e-mail and letter correspondence observations. Here, we demonstrate that, like e-mail correspondence, the letter correspondence patterns of 16 writers, performers, politicians, and scientists are well-described by the circadian cycle, task repetition and changing communication needs. We confirm the universality of these mechanisms by properly rescaling letter and e-mail correspondence statistics to reveal their underlying similarity.

==> methods.tex <==
%=====================================================================
%=====================================================================
%=====================================================================
% METHODS
%=====================================================================
%=====================================================================
%=====================================================================
\section*{Methods}

%=====================================================================
% model predictions
%=====================================================================

% analytic solution to p(tau)
Consider a \cpp~with parameters $\bftheta=\{\rate,\q\}$.  The inter-event
time distribution is given by
%
\begin{eqnarray}
\condprob{\tau}{\bftheta} & = & \left\{
\begin{array}{ll}
\q & \tau = 0 \\
(1-\q)\rate e^{-\rate \tau} & \tau > 0 \\
\end{array}
\right. ,
\label{eqn:tau}
\end{eqnarray}
%
and the probability of observing $\NT$ events during a time interval of
duration $\TT$ can be written as
%
\begin{equation}
\condprob{\NT}{\bftheta} =
\begin{cases}
e^{-\rate \TT} & \NT = 0 \\
e^{-\rate \TT} \Qntheta{\NT-1} & \NT > 0 \\
\end{cases}
\,,
\label{eqn:nt}
\end{equation}
%
where the polynomial 
%
\begin{eqnarray}
\Qntheta{\NN} & = & (1-\q)\rate\TT
\sum_{\nnn=0}^{\NN} \binom{\NN}{\nnn}
\frac{\q^{\nnn} \left[(1-\q)\rate\TT\right]^{\NN-\nnn}}{(\nnn+1)!}
\label{eqn:q}
\end{eqnarray}
%
accounts for the various ways that the $\NN=\NT-1$ events during the time
interval of duration $\TT$ time units can be grouped into cascades of activity.
The censored likelihood function is given by
%
\begin{eqnarray}
\mathcal{L}(\bftheta) & = &\prod_{\kkk=0}^{\T/\TT-1}
\condProb{\NN_{\TT,\kkk}}{\bftheta} ,
\label{eqn:ll}
\end{eqnarray}
%
where $\T$ is the duration of the time segment, $\TT=1$ day, and
$\NN_{\TT,\kkk}$ is the number of events that occur on day $\kkk$.  The
derivation for these quantities can be found in \secref{\cppanalsec}.


